Discovery of 28 pulsars using new techniques for sorting pulsar candidates

Modern pulsar surveys produce many millions of candidate pulsars, far more than can be individually inspected. Traditional methods for filtering these candidates, based upon the signal-to-noise ratio of the detection, cannot easily distinguish between interference signals and pulsars. We have developed a new method of scoring candidates using a series of heuristics which test for pulsar-like properties of the signal. This significantly increases the sensitivity to weak pulsars and pulsars with periods close to interference signals. By applying this and other techniques for ranking candidates from a previous processing of the Parkes Multi-beam Pulsar Survey, 28 previously unknown pulsars have been discovered. These include an eccentric binary system and a young pulsar which is spatially coincident with a known supernova remnant.

==> profiles/123.tex <==
J1055$-$6028 & 4.73 & 12.24 & 36.08 & 30.0 & 15.1 & $-$0.39 & $-$0.20 & 702.0 & 178.5\\ 
J1244$-$6531 & 6.53 & 12.53 & 31.89 & 30.0 & 9.4 & $-$1.39 & $-$0.44 & 153.0 & 15.0\\ 
J1321$-$5922 & 6.93 & 12.25 & 31.65 & 23.0 & 9.0 & 1.31 & 0.51 & 100.2 & 15.4\\ 
J1433$-$6038 & 6.74 & 12.53 & 31.48 & 9.9 & 6.3 & $-$0.03 & $-$0.02 & 22.8 & 9.1\\ 
J1518$-$5415 & 7.92 & 10.98 & 32.20 & 4.3 & 3.2 & 0.20 & 0.15 & 1.5 & 0.8\\ 
\\
J1524$-$5819 & 5.08 & 13.05 & 33.75 & 10.9 & 6.2 & $-$0.23 & $-$0.13 & 10.6 & 3.4\\ 
J1536$-$5907 & 6.81 & 11.95 & 32.49 & 12.0 & 6.0 & $-$0.57 & $-$0.29 & 31.5 & 7.9\\ 
J1538$-$5519 & 8.19 & 11.11 & 31.41 & 9.8 & 7.5 & 0.02 & 0.02 & 40.4 & 23.7\\ 
J1636$-$4440 & 4.85 & 12.50 & 35.32 & 9.5 & 6.6 & 0.30 & 0.21 & 34.4 & 16.4\\ 
J1637$-$4816 & 6.36 & 12.35 & 32.59 & 10.0 & 8.5 & $-$0.14 & $-$0.12 & 74.0 & 53.0\\ 
\\
J1654$-$4245 & 5.53 & 12.88 & 33.18 & 11.8 & 10.9 & 0.12 & 0.11 & 19.6 & 16.6\\ 
J1702$-$4306 & 5.54 & 12.17 & 34.59 & 7.1 & 6.7 & $-$0.10 & $-$0.09 & 13.8 & 12.0\\ 
J1715$-$3247 & 8.34 & 11.54 & 30.26 & 4.0 & 3.2 & 0.23 & 0.18 & 1.3 & 0.8\\ 
J1716$-$4111 & 6.76 & 12.24 & 32.00 & 4.8 & 4.0 & $-$0.15 & $-$0.12 & 5.0 & 3.5\\ 
J1747$-$2647 & 5.78 & 12.41 & 33.62 & 8.3 & 7.3 & 0.11 & 0.10 & 105.8 & 81.8\\ 
\\
J1753$-$2240 & 9.28 & 9.94 & 31.56 & 3.5 & 3.0 & 0.10 & 0.09 & 1.8 & 1.4\\ 
J1755$-$2025 & 6.06 & 12.08 & 33.72 & 8.7 & 6.4 & 0.37 & 0.27 & 13.6 & 7.4\\ 
J1756$-$2619 & 6.97 & 11.98 & 32.11 & 7.5 & 7.1 & $-$0.12 & $-$0.11 & 5.7 & 5.0\\ 
J1818$-$1556 & 7.33 & 11.92 & 31.51 & 4.1 & 3.9 & $-$0.02 & $-$0.02 & 8.1 & 7.6\\ 
J1821$-$1432 & 6.75 & 12.51 & 31.48 & 7.5 & 7.0 & $-$0.02 & $-$0.02 & 12.5 & 10.9\\ 
\\
J1830$-$1313 & 6.84 & 12.06 & 32.20 & 10.4 & 8.0 & $-$0.27 & $-$0.21 & 28.3 & 16.6\\ 
J1840$-$0626 & 6.11 & 12.82 & 32.11 & 9.2 & 8.9 & $-$0.07 & $-$0.07 & 13.5 & 12.6\\ 
J1843$-$0744 & 5.75 & 12.40 & 33.69 & 5.7 & 5.6 & $-$0.17 & $-$0.16 & 5.5 & 5.4\\ 
J1846$-$0749 & 6.42 & 12.33 & 32.51 & 4.4 & 3.9 & $-$0.18 & $-$0.16 & 3.7 & 2.9\\ 
J1850$-$0006 & 6.91 & 12.49 & 31.20 & 7.2 & 8.0 & 0.01 & 0.01 & 41.9 & 50.7\\ 
\\
J1850$-$0026 & 4.83 & 12.41 & 35.52 & 11.2 & 10.8 & 0.01 & 0.01 & 222.9 & 205.7\\ 
J1851$-$0029 & 6.24 & 12.20 & 33.11 & 6.9 & 7.6 & $-$0.04 & $-$0.04 & 20.8 & 25.2\\ 
J1855+0527 & 4.92 & 13.29 & 33.59 & 9.8 & 7.9 & 0.28 & 0.23 & 23.0 & 15.1\\ 


==> profiles/npsrs.tex <==
\def\npsrs{28}

